Ambient Adventures: Teaching ChatGPT on Developing Complex Stories

Imaginative play is an area of creativity that could allow robots to engage with the world around them in a much more personified way. Imaginary play can be seen as taking real objects and locations and using them as imaginary objects and locations in virtual scenarios. We adopted the story generation capability of large language models (LLMs) to obtain the stories used for imaginary play with human-written prompts. Those generated stories will be simplified and mapped into action sequences that can guide the agent in imaginary play. To evaluate whether the agent can successfully finish the imaginary play, we also designed a text adventure game to simulate a house as the playground for the agent to interact.

==> tables/realworldsteps.tex <==
\begin{table}[h]
\centering
\footnotesize
\setlength\tabcolsep{0.1pt} %
\begin{tabular}{p{0.99\linewidth}}
\toprule
\textbf{Real-World Translation Example:} 1. Wear clothes 2. Open nightstand 3. Go south 4. Go east 5. Use broom 6. Go west 7. Go north 8. Open dresser 9. Go south 10. Go east. 11. Use broom 12. Go west 13. Go north 14. Open dresser 15. Go south 16. Go east 17. Use broom
\bottomrule
\end{tabular}
\caption{Real-World Translation With Navigation
}
\label{tab:ex_navigation_chatgpt}
\end{table}
